Positive Experience Reflection for Agents in Interactive Text Environments

Intelligent agents designed for interactive environments face significant challenges in text-based games, a domain that demands complex reasoning and adaptability. While agents based on large language models (LLMs) using self-reflection have shown promise, they struggle when initially successful and exhibit reduced effectiveness when using smaller LLMs. We introduce Sweet&Sour, a novel approach that addresses these limitations in existing reflection methods by incorporating positive experiences and managed memory to enrich the context available to the agent at decision time. Our comprehensive analysis spans both closed- and open-source LLMs and demonstrates the effectiveness of Sweet&Sour in improving agent performance, particularly in scenarios where previous approaches fall short.

==> sections/related.tex <==
\section{Related Work}
\subsection{Controlling LLMs \& Their Memory}
Recently, several approaches to managing LLM memory in general contexts have been proposed~\citep{packer2023memgpt, wang2023augmenting}.
%
%\citet{packer2023memgpt} propose a framework employing a decoupled network architecture with a frozen original LLM backbone as a memory encoder and an adaptive residual side-network as a memory retriever and reader, facilitating the memorization of long history without suffering from memory staleness
%
%\citet{wang2023augmenting} propose virtual context management, drawing inspiration from hierarchical memory systems, to extend context within the LLM's window and efficiently manage different memory tiers.
%
The limitation of memory in LLMs due to limited context windows becomes particularly apparent in summarization tasks.
%
One approach to tackle this is through recursive summarization where the LLM generates concise representations over a sliding window to fit them within a specified token length~\citep{wu2021recursively}.
%
This summarization process is inherently lossy and can lead to the unintentional loss of relevant details.
%
\citet{adams2023sparse} propose Chain of Density, an iterative summarization technique for news articles which progressively makes the generated summary more salient entity-dense without increasing its length.
%
Our summarization approach differs from theirs as we tackle a non-static problem, \emph{i.e.} we effectively summarize evolving content across time steps.







